A Unified Memory Perspective for Probabilistic Trustworthy AI

Trustworthy artificial intelligence increasingly relies on probabilistic computation to achieve robustness, interpretability, security and privacy. In practical systems, such workloads interleave deterministic data access with repeated stochastic sampling across models, data paths and system functions, shifting performance bottlenecks from arithmetic units to memory systems that must deliver both data and randomness. Here we present a unified data-access perspective in which deterministic access is treated as a limiting case of stochastic sampling, enabling both modes to be analyzed within a common framework. This view reveals that increasing stochastic demand reduces effective data-access efficiency and can drive systems into entropy-limited operation. Based on this insight, we define memory-level evaluation criteria, including unified operation, distribution programmability, efficiency, robustness to hardware non-idealities and parallel compatibility. Using these criteria, we analyze limitations of conventional architectures and examine emerging probabilistic compute-in-memory approaches that integrate sampling with memory access, outlining pathways toward scalable hardware for trustworthy AI.

==> backup.tex <==
\begin{comment}

\noindent Artificial intelligence systems are increasingly deployed in high-stakes settings, from medical decision-making~\cite{isscc_shot_noise,abdelrazikWearableDevicesArrhythmia2025,metwallyPredictionMetabolicSubphenotypes2025,diazcPerformanceBasedAdaptationIndex2025} to autonomous platforms~\cite{yuCooperativePathPlanning2015,automated_driving_nn,autonomous_driving_dl} and robotic agents~\cite{science_robotics_uhang,robot_embodied_ai_2021,robot_arm_2025}. In these regimes, uncertainty is not a peripheral disturbance but a structural feature of the problem: inputs are noisy, environments evolve, and models are imperfect or adversarially exposed. Trustworthy operation therefore demands more than correctness—it requires calibrated confidence, interpretability and controlled information exposure. The computational objective shifts from producing point predictions to managing and propagating uncertainty.

This transition moves AI computation from function space to distribution space. Rather than evaluating a deterministic mapping $y = f(x)$, trustworthy systems must estimate expectations, quantify risk, assess rare events and compare distributions. Uncertainty quantification~\cite{uncertainty,peiUncertaintyawareRoboticPerception2025a,nutiExplainableBayesianDecision2021} provides a canonical example: predictive statistics take the form
\begin{equation}
\mathbb{E}_{p(w|D)}[f(x,w)] = \int f(x,w)\, p(w|D)\, dw ,
\end{equation}
which, in high-dimensional nonlinear and non-Gaussian models, rarely admits closed-form solutions. Deterministic quadrature methods scale poorly with dimension, making sampling a dimension-robust estimator. Other trust mechanisms—including perturbation-based interpretability~\cite{ribeiro_lime_2016,lundberg_shap_2017} and privacy-preserving schemes based on controlled randomness~\cite{dworkAlgorithmicFoundationsDifferential2014,liuPrivacybySensingTimedomainDifferentiallyPrivate2023,davisInSituPrivacyMixedSignal2024,caoStochasticMixedSignalCircuit2022a}—differ mathematically, yet similarly rely on repeated sampling and entropy generation. Across these settings, sampling becomes a defining workload characteristic.

Rather than addressing broader socio-ethical and governance questions~\cite{ec-ethics-trustworthy-ai-2018,DARPA_xai_2019,nist-trust-ai,gao-ai-accountability-2021}, this Perspective focuses on the computational substrate of trustworthy AI. We examine how distribution-level reasoning reshapes workload structure and argue that entropy-intensive operation has direct architectural implications, particularly for memory systems.




Prior reviews~\cite{distribution_conversion,ghahramani_probabilistic_2015,wang_safe_2024} have examined diverse algorithms and emerging devices for probabilistic computation, as well as certain perspectives of hardware trustworthiness, such as security of compute-in-memory. However, comparatively little attention has been paid to how probabilistic workloads—spanning different models, sampling regimes, and trust objectives—interact with and stress hardware systems, particularly memory. In practice, trustworthy AI workloads interleave deterministic data access with repeated sampling, causing memory systems to emerge as a primary bottleneck and creating hybrid access patterns that challenge conventional memory hierarchies.

\end{comment}

\begin{comment}
    \noindent\textbf{Workload Structure and Memory Stress}

\noindent When viewed from a systems perspective, trustworthy AI workloads share a recurring pattern: sampling permeates multiple stages of computation rather than appearing as a single isolated step.

At the model level, uncertainty-aware inference repeatedly samples parameters, tightly coupling stochastic generation with parameter memory access (e.g., Bayesian neural networks~\cite{liu15365nmUncertaintyQuantifiable2025,peiUncertaintyQuantifiableBiomedicalIntelligence2025}). A similar coupling arises in probabilistic embedding search, where similarity evaluation operates over distribution-valued representations and sampling is intrinsically bound to embedding reads. At the feature level, latent-variable models sample internal representations (e.g., variational autoencoders~\cite{variational_inference1,kingmaAutoEncodingVariationalBayes2022}). At the data level, interpretability methods estimate conditional expectations via randomized perturbations (e.g., LIME or SHAP~\cite{ribeiro_lime_2016,lundberg_shap_2017}), generating streaming input accesses while repeatedly querying model parameters. In generative settings~\cite{kingmaAutoEncodingVariationalBayes2022,hoDenoisingDiffusionProbabilistic2020}, iterative sampling sustains entropy demand across refinement steps.

Privacy and security mechanisms introduce further stochastic pressure. Differential privacy injects controlled noise~\cite{dworkAlgorithmicFoundationsDifferential2014,liuPrivacybySensingTimedomainDifferentiallyPrivate2023,davisInSituPrivacyMixedSignal2024,caoStochasticMixedSignalCircuit2022a}, probabilistic watermarking embeds statistical signatures into output distributions~\cite{llm_watermark}, and in-memory encryption in CIM or non-volatile systems requires high-throughput or high-quality entropy sources to protect models and data. Although differing in objective, these mechanisms impose repeated stochastic operations with strict randomness requirements.

Across these scenarios, deterministic memory accesses are interleaved with sampling and entropy generation, creating hybrid access patterns fundamentally distinct from purely deterministic workloads. As sampling frequency increases, both memory subsystems and random number generation become co-critical resources, motivating a quantitative measure of how tightly entropy consumption is coupled to memory activity.




\noindent\textbf{Formal Abstraction of Probabilistic Memory}

\noindent To analyze these workloads systematically, we adopt a unified memory abstraction.

In conventional systems, memory performs deterministic mapping:
\begin{equation}
\mathcal{M}_{\text{det}}(a) \rightarrow x ,
\end{equation}
where address $a$ returns a stored value $x$.

In probabilistic workloads, memory access is coupled with sampling. We extend the abstraction as
\begin{equation}
\mathcal{M}_{\text{prob}}(a,\theta) \rightarrow X \sim P_\theta ,
\end{equation}
where distribution parameters $\theta$ are stored in memory and a read returns a sample drawn from $P_\theta$.

Under this formulation, deterministic memory becomes a limiting case in which
\begin{equation}
\mathrm{Var}(X) \rightarrow 0 .
\end{equation}

Sampling thus becomes a first-class memory operation rather than a peripheral software routine. Memory mediates not only stored values but also entropy and distributional semantics.


\noindent\textbf{Entropy Intensity}

\noindent Under this abstraction, entropy consumption becomes a structural workload property rather than an implementation detail. We define entropy intensity as
\begin{equation}
EI = \frac{H_{\text{consumed}}}{B_{\text{memory}}},
\end{equation}
where $H_{\text{consumed}}$ denotes entropy bits consumed during stochastic operations and $B_{\text{memory}}$ denotes memory bits accessed during execution. Entropy intensity quantifies how tightly randomness is coupled to memory activity.

Three regimes naturally emerge. In \textbf{low-EI regimes} ($EI \approx 0$), entropy is used only occasionally—such as during model initialization, sporadic dropout, or one-time encryption—and remains negligible relative to memory traffic. Computation is effectively deterministic, and conventional memory hierarchies suffice.

In \textbf{intermediate-EI regimes} ($0 < EI < 1$), stochastic operations are present but subordinate to parameter or data movement. Entropy consumption grows more slowly than memory access, as in variational autoencoders where latent sampling is followed by large deterministic decoders, or in Monte Carlo similarity evaluation where sampling is amortized over substantial model reads.

In \textbf{high-EI regimes} ($EI = O(1)$), entropy generation scales proportionally with memory access. Each parameter or data read is intrinsically associated with stochastic processing, as in Bayesian neural networks, probabilistic embedding search, differential privacy with per-element noise injection, or fine-grained in-memory protection mechanisms. In such regimes, entropy delivery, statistical quality, and randomness locality become first-order architectural constraints.



\noindent\textbf{Evaluation Criteria}

\noindent Motivated by this abstraction, we identify five criteria for evaluating memory systems under entropy-intensive workloads:

(C1) Unified deterministic–probabilistic semantics: read, write, and sample operations are supported coherently within a unified abstraction.

(C2) Distribution programmability: memory enables flexible configuration of distribution parameters (e.g., mean, variance, mixture weights) without architectural specialization.

(C3) Hardware efficiency: throughput, energy, and density scale with sampling intensity.

(C4) Robustness to non-idealities: sampling statistics remain stable under process variation, voltage fluctuation, temperature shifts, aging, and radiation.

(C5) Parallel compatibility: probabilistic operations integrate naturally with parallel AI accelerators without introducing correlation or serialization bottlenecks.

Together, these criteria provide a structured framework for analyzing how conventional von Neumann architectures and emerging probabilistic compute-in-memory approaches support entropy-intensive AI workloads.
\end{comment}
    

\begin{comment}


\noindent \textbf{Unified Semantic}
 

Because sampling recurs across models, data paths, and system functions—with widely varying frequency, locality, and duration—stage-specific or ad hoc handling becomes increasingly untenable. At the software level, probabilistic semantics are already first-class, allowing uncertainty to be expressed directly through distribution-valued variables and sampling primitives (for example, in probabilistic programming frameworks such as PyMC). However, current memory systems continue to treat sampling as a peripheral operation, leading to fragmented execution paths and inefficient utilization when deterministic and probabilistic accesses are tightly interleaved. This motivates an evaluation metric that assesses how well a memory architecture natively supports read, write, and sample as first-class operations, providing a unified semantic foundation that aligns hardware behavior with software-level representations of uncertainty in trustworthy AI.

\noindent\textbf{Distribution Programmability}

\noindent Distribution programmability extends the notion of conventional data programmability to probabilistic representations. In addition to storing deterministic values, probabilistic memory must support the configuration of distributional parameters—such as mean, variance, or mixture weights—without requiring architectural reconfiguration or algorithm-specific post-processing. This capability is essential because different probabilistic AI models rely on distinct distributional forms that directly shape memory access patterns and sampling intensity. This capability is essential because different probabilistic AI models rely on distinct distribution forms that directly shape memory access behavior. Gaussian distributions with tunable mean and variance underpin Bayesian neural networks and variational inference, encoding uncertainty in weights or activations. Laplacian distributions are commonly adopted in sparse Bayesian models and robustness-oriented formulations that emphasize sharp deviations or heavy-tailed behavior~\cite{laplacian_sparse_bayesian,Sparse_Bayesian_Classification}. Uniform distributions appear in randomized exploration, initialization, and sampling-based perturbation methods used for explainability and uncertainty probing~\cite{mog_uniform, ribeiro_lime_2016}. Bimodal and multimodal distributions arise naturally in mixture models and Bayesian formulations that capture competing hypotheses or ambiguous inputs~\cite{coutinual_learning, mix_of_two_gaussian}. Treating probabilistic data as first-class memory content therefore requires flexible control over these distributional properties, rather than reliance on fixed or implicit randomness. From a memory-level perspective, such programmability is a fundamental capability, allowing a single memory substrate to support diverse probabilistic models in much the same way that conventional memory supports heterogeneous deterministic data.
Efficiency and Robustness

\noindent\textbf{Efficiency and Robustness}

Alongside programmability, hardware efficiency and sampling robustness impose equally stringent constraints on probabilistic memory systems. Many trustworthy AI agents operate under strict physical limits in real-world settings, such as implantable medical devices or autonomous platforms deployed in harsh environments, where computation must be executed in real time under tight power and area budgets. As sampling intensity increases, these workloads place direct demands on memory systems to deliver high throughput, high energy efficiency, and high density without degrading the statistical quality of generated samples. Robustness to hardware non-idealities—including process, voltage, and temperature (PVT) variations, aging and endurance effects, and radiation-induced errors—is therefore critical, as such effects can distort sampling distributions and bias probabilistic inference, particularly in edge deployments where recalibration is often impractical. Compatibility with parallel execution is also essential, since modern edge AI accelerators rely on concurrency to meet performance targets; probabilistic memory operations must support simultaneous access and sampling without introducing correlation or serialization artifacts. Together, these considerations underscore the need for probabilistic memory systems that preserve sampling quality while remaining efficient, scalable, and robust by design.


\noindent\textbf{Evaluation Criteria}


\noindent Motivated by the discussion above, we identify five memory-level criteria that are useful for evaluating how memory systems support probabilistic workloads in machine learning, and use them to organize the remainder of this Perspective. (C1) memory systems can be assessed by whether probabilistic and deterministic accesses are supported in a unified manner for both write and read or sampling operations, treating probabilistic data as a first-class extension of conventional memory rather than as a separate primitive. (C2) distribution programmability provides a key dimension of comparison, reflecting how conveniently distribution shapes and parameters can be configured, analogous to deterministic data writes, without relying on specialized hardware paths or incurring excessive overhead. (C3) Hardware efficiency—encompassing throughput, energy, and area—becomes a critical metric as probabilistic operations scale with sampling intensity under tight resource constraints. (C4) Sampling statistical quality is robust to hardware non-idealities, including process variation, voltage fluctuation, temperature changes as well as aging, endurance and radiation, is essential for maintaining stable probabilistic behavior without frequent calibration. (C5) Finally, compatibility with parallel AI computation distinguishes memory systems that align naturally with modern parallel accelerators from those that serialize probabilistic operations. Together, these criteria form a unified framework for analyzing and comparing probabilistic memory systems in the context of trustworthy AI.
\end{comment}

\begin{comment}

\noindent\textbf{Throughput density mismatch}

\noindent Hardware implementations reveal a growing mismatch between the throughput density of random number generation and modern compute fabrics. Highly optimized digital GRNG implementations typically achieve sampling throughputs on the order of $10^{8}$--$10^{9}$ samples per second per instance~\cite{thomasGaussianRandomNumber2007a,malikGaussianRandomNumber2016}. When normalized by silicon area, the achievable throughput density generally falls in the range of approximately $10^{6}$--$10^{9}$ samples s$^{-1}$ mm$^{-2}$.

In contrast, modern AI compute platforms achieve dramatically higher computation densities. Through massive parallelism and increasingly through computing-in-memory architectures, state-of-the-art accelerators can reach effective compute densities on the order of $10^{2}$--$10^{4}$ TOPS mm$^{-2}$~\cite{khwa34216nm96Kb2024,shih201NVE3nm2024,khwa14216nm216kb2025}. This large disparity creates a fundamental mismatch between arithmetic capability and stochastic data generation, as shown in Fig.~\ref{fig:bottleneck}(a). As compute throughput density continues to scale, the relative cost of sampling grows accordingly, making random number generation an increasingly important system bottleneck for high sampling-intensity workloads.

\noindent\textbf{Sampling intensity and algorithm regimes}

\noindent To understand how this mismatch affects algorithms, it is useful to consider the \textit{sampling intensity} of a workload. Sampling intensity describes how frequently stochastic sampling occurs relative to deterministic computation or memory access. In workloads with low sampling intensity, sampling occurs only occasionally and has limited impact on system performance. In contrast, workloads with high sampling intensity repeatedly perform stochastic sampling as part of normal execution.

As sampling intensity increases, the demand for random samples grows proportionally with algorithm complexity, model size, or iteration count. In such regimes, system performance can transition from being limited by deterministic computation or memory access to being limited by the throughput of random number generation. When the sampling intensity exceeds the relative throughput gap between computation or memory and RNG generation, system performance becomes bounded by RNG throughput.

For example, Bayesian neural networks typically exhibit very high sampling intensity with respect to both computation and memory. For each weight access or MAC operation, random sampling is often required, such as generating Gaussian-distributed weights during inference. Similar behavior appears in probabilistic embedding search, differential privacy mechanisms, and Monte Carlo integration. In contrast, diffusion models, despite requiring significant randomness, are often dominated by computation or memory traffic because the number of MAC operations and memory accesses can greatly exceed the number of random samples required.

Fig.~\ref{fig:bottleneck}.(b) illustrates a projection of sampling intensity with respect to both computation and memory across representative algorithms. The gap between compute throughput density and GRNG throughput density continues to widen, particularly with the emergence of computing-in-memory architectures that further increase compute density.

These observations suggest that, for a growing class of probabilistic workloads, random number generation has become a first-order system bottleneck in conventional von Neumann architectures.
    \noindent\textbf{Random Number Generation Algorithms}

\noindent In conventional von Neumann systems, probabilistic computation relies on explicit random number generation pipelines that are largely decoupled from memory access. Most implementations follow a two-stage structure: uniform random number generation (URNG), typically realized using linear congruential generators~\cite{knuth1997art,coutureLatticeStructureCertain1994}, Mersenne Twister variants~\cite{matsumotoMersenneTwister623dimensionally1998}, XOR-shift generators~\cite{pannetonXorshiftRandomNumber2005}, or counter-based schemes~\cite{salmonParallelRandomNumbers2011}, followed by distribution shaping to obtain Gaussian or other target distributions. URNG itself can achieve very high bit rates at low cost, but generating non-uniform distributions—particularly Gaussian random number generation (GRNG)—is of greater practical interest and is substantially more hardware-expensive. 

As one of the most widely used distribution priors, Gaussian sampling is commonly implemented using algorithms such as Box–Muller~\cite{boxNoteGenerationRandom1958}, Ziggurat~\cite{marsagliaZigguratMethodGenerating2000}, and transform-based methods (e.g., Wallace~\cite{wallaceFastPseudorandomGenerators1996}). Box–Muller offers high statistical quality but requires multiple transcendental operations, leading to deep pipelines and high latency. Ziggurat reduces average computation through table-driven acceptance–rejection, but introduces irregular control flow and memory lookups. Transform-based methods amortize computation across batches of samples, but require buffering and careful correlation management. Across these approaches, algorithmic complexity grows rapidly with sampling rate, making GRNG substantially more expensive than deterministic arithmetic as sampling intensity increases.

Sampling from arbitrary distributions further increases algorithmic and architectural complexity in conventional systems. Such distributions are typically generated by transforming uniform random numbers using inverse-CDF, rejection, or table-based methods. These approaches incur substantial computation and memory overhead, introduce data-dependent control flow and variable latency, and reduce predictability and parallel efficiency. As distribution fidelity, dimensionality, or sampling rate increases, arbitrary distribution sampling becomes increasingly expensive relative to deterministic arithmetic.

\noindent\textbf{Hardware Implementations}

\noindent State-of-the-art hardware implementations illustrate that, even for widely studied target distributions such as Gaussian, high absolute sampling throughput can be achieved only through aggressive pipelining and spatial replication. Deeply pipelined digital GRNGs report per-instance throughputs on the order of $10^{8}$--$10^{9}$ Gaussian samples per second\cite{thomasGaussianRandomNumber2007a,malikGaussianRandomNumber2016}, while multi-instance designs can scale into the multi-billion-sample-per-second regime at the cost of substantial area and power overhead\cite{curand}. When normalized by silicon area, however, achievable GRNG throughput density remains limited to approximately $10^{6}$--$10^{9}$ samples~s$^{-1}$~mm$^{-2}$, even in highly optimized ASIC and FPGA implementations. In contrast, contemporary AI compute fabrics routinely achieve effective computation densities of $10^{2}$--$10^{4}$~TOPS~mm$^{-2}$ by exploiting in memory computation\cite{khwa34216nm96Kb2024, shih201NVE3nm2024, khwa14216nm216kb2025}. Mixed-signal and noise-based GRNGs have also been explored to improve efficiency by leveraging thermal noise\cite{johnsonThermalAgitationElectricity1928,stipcevicFastNondeterministicRandom2004}, jitter\cite{yooImprovingRobustnessRing2010}, or device mismatch\cite{enciso65NmBayesian2025a}, but these approaches often require analog biasing, calibration, or digital post-processing to maintain statistical quality, limiting robustness and scalability. Moreover, in von Neumann systems, generated samples are materialized as explicit digital values that must be written to and read from registers or memory, further amplifying bandwidth and energy costs and constraining parallel execution.

\noindent\textbf{Probabilistic Bandwidth Bottlenecks}

\noindent Together, these results expose a fundamental throughput-density mismatch between GRNG and computation in von Neumann architectures. While arithmetic throughput density has scaled aggressively with technology and architectural parallelism, GRNG throughput density lags behind by four to six orders of magnitude, making sampling a first-order bottleneck in probabilistic workloads. As sampling intensity increases, such as in Bayesian inference, Monte Carlo uncertainty estimation, or diffusion-based training, systems rapidly transition from being compute-bound to being dominated by sampling and data movement. This imbalance is particularly acute in edge deployments, where power and area budgets prohibit large-scale GRNG replication and where latency constraints limit deep pipelining. More fundamentally, the von Neumann paradigm enforces a separation between memory, computation, and sampling, treating samples as external data streams rather than intrinsic properties of memory access. As a result, incremental optimization of GRNG algorithms or circuits alone cannot close this gap, highlighting a structural limitation of von Neumann architectures for high-rate probabilistic dataflows.

\end{comment}

\begin{comment}
    \noindent\textbf{What is probabilistic compute-in-memory?}

\noindent The limitations of von Neumann architectures arise from compounded bottlenecks in computation, memory access, and random number generation. Although compute-in-memory (CIM) alleviates memory bandwidth and data-movement costs for deterministic workloads, combining CIM with faster or more efficient random number generators does not fundamentally resolve probabilistic workload. As long as sampling remains an external operation—materialized as explicit random numbers and injected into computation—the system continues to suffer from sampling throughput limits, excess memory traffic, and restricted parallelism.
Probabilistic compute-in-memory (p-CIM) addresses this limitation by integrating sampling directly into memory operations. Rather than treating randomness as a separate data stream, p-CIM embeds probabilistic behavior into how memory is accessed or updated, allowing sampling activity to scale with memory bandwidth and spatial parallelism. By avoiding the explicit generation, storage, and transport of random numbers, p-CIM targets the system-level inefficiencies that dominate probabilistic workloads within a unified memory-centric framework.
From a memory-level perspective, p-CIM extends conventional memory semantics to support probabilistic access alongside deterministic operations. Deterministic reads can be interpreted as a limiting case in which variance collapses to zero, whereas probabilistic reads yield samples drawn from device-defined or programmable distributions. Importantly, this abstraction does not enforce identical semantics across all implementations: different p-CIM designs balance intrinsic sampling efficiency, programmability, and compatibility with deterministic access in different ways. This flexibility motivates the distinction between coupled and decoupled p-CIM architectures, discussed in the following sections.



\noindent\textbf{CMOS Entropy Sources}

\noindent In probabilistic compute-in-memory systems, entropy sources must be compatible with dense memory integration and support repeated, parallel sampling during memory access. Within conventional CMOS technologies, a wide range of entropy-generation mechanisms has been explored, primarily leveraging either dynamic circuit noise or static device variability.


Dynamic entropy sources exploit intrinsic electronic noise, including thermal noise\cite{res_noise} and shot noise\cite{isscc_shot_noise,JSSC_shot_noise}, which can be captured through current integration or capacitor charging and converted into voltage- or time-domain signals suitable for sampling. Time-domain uncertainty provides another widely used mechanism: phase jitter in ring oscillators or delay lines\cite{rint_osc,couple_osc,ring_power_noise_rng} can be digitized through sampling or edge counting, while metastability-based approaches\cite{Metastability} drive bistable circuits into unstable states where intrinsic noise resolves the final logic value. In addition, static entropy sources exploit fabrication-induced device mismatch or leakage-current variation\cite{pv1,pv2,pv3}, amplifying these variations during sensing to generate reproducible but device-unique random behavior.


A key advantage of CMOS-based entropy sources is their compatibility with standard processes, mature design flows, and robust digital integration, which aligns well with the requirements of programmable and reliable pCIM architectures. However, the intrinsic amplitude of CMOS noise mechanisms is typically small, requiring dedicated amplification, averaging, or auxiliary circuitry to achieve usable randomness. As a result, multiple transistors or peripheral circuits are often needed to generate a single effective entropy source, leading to limited entropy density when tightly integrated within memory arrays. Moreover, both dynamic and static CMOS entropy sources exhibit sensitivity to process, voltage, and temperature variations, which frequently necessitates calibration, post-processing, or architectural mitigation to maintain stable probabilistic behavior.


These characteristics make CMOS entropy sources technology-ready and robust, but also highlight a fundamental density and efficiency challenge when scaling probabilistic compute-in-memory toward high-throughput, massively parallel sampling. This motivates the exploration of emerging memory and device technologies that offer stronger intrinsic stochasticity at the single-device level, which we discuss next.

\noindent\textbf{Emerging Entropy Sources Beyond CMOS}

\noindent While CMOS-compatible entropy sources benefit from mature processes and robust integration, their entropy density is ultimately constrained by small-amplitude noise mechanisms that typically require multiple transistors and peripheral circuitry\cite{electrical_noise_review}. This limitation motivates a shift toward stochastic physical mechanisms intrinsic to memory and device operation, in which randomness arises directly from switching or transport processes\cite{distribution_conversion}. Examples include resistive switching in ReRAM\cite{Memristors_review,memristor_bitstream,memristors_review2}, thermally driven phase transitions in PCM\cite{pcm}, probabilistic magnetization reversal in spin-transfer torque magnetic devices\cite{mram_rng,mram_rng2,mram_rng3}, stochastic polarization switching in ferroelectric transistors\cite{fefet_cim}, floating-body and impact-ionization effects in FDSOI technologies\cite{peiUncertaintyawareRoboticPerception2025a}, and quantum or spontaneous-emission noise in photonic platforms\cite{photonic_ase_rng,photonic_quantum_vacuum_bnn,photonic_review}. In these systems, randomness is not a secondary perturbation but an inherent consequence of device physics, enabling higher entropy per device and tighter spatial colocation of storage and sampling within memory arrays.


At a high level, such entropy sources can be realized through two distinct modes of operation\cite{writing_reading}. Read-based mechanisms extract randomness during sensing or readout, favoring energy efficiency and device lifetime but typically offering limited and indirect control over the resulting distribution. Write-based mechanisms generate randomness through stochastic programming or switching events, providing stronger stochasticity and a wider achievable distribution range, at the cost of higher write energy and potential endurance concerns\cite{endurance}. This recurring efficiency–lifetime versus programmability trade-off shapes how device-level entropy can be incorporated into probabilistic compute-in-memory systems and motivates architectural strategies that balance entropy generation with distribution control, as discussed in the following sections.

\noindent\textbf{Coupled Parameter Storage and Sampling}

\noindent Probabilistic compute-in-memory requires that both parameter storage and sampling be supported within the memory system, enabling probabilistic values to be generated and consumed without leaving the memory hierarchy. Emerging non-volatile memory devices naturally satisfy this requirement by providing stochastic physical mechanisms intrinsic to their operation, allowing sampling to be embedded directly into memory access.


Coupled pCIM architectures exploit this property by realizing parameter storage and sampling within the same physical device\cite{Memristors_bayesian_review}. In such designs, probabilistic behavior emerges directly during read or write operations, leveraging device-level stochasticity without explicit random number generation. Collapsing storage and entropy generation into a single device-level operation aligns sampling throughput with array-level parallelism and minimizes data movement, resulting in high energy efficiency, compact area, and low latency. These characteristics make coupled pCIM particularly attractive for workloads with high sampling intensity.


In practice, coupled pCIM implementations follow either read-based or write-based sampling, exposing a fundamental efficiency–programmability trade-off. Read-based coupling extracts randomness during sensing without modifying stored parameters. ReRAM-based pCIM exemplifies this approach\cite{rram_cim,writing_reading_application}: stochastic read-current fluctuations associated with filamentary conduction introduce randomness during read operations, while programmed conductance values set the nominal mean and spatial aggregation (number of devices) shapes the variance. This strategy benefits from low energy consumption and long device lifetime, but distribution control remains coarse and strongly constrained by device physics, often requiring additional hardware resources to extend the achievable variance range.


Write-based coupling, in contrast, generates randomness through stochastic programming or switching events\cite{rram_write,rram_write2}. FeFET-based pCIM illustrates this mode of operation\cite{fefet_cim}, where incremental step pulse programming induces stochastic threshold-voltage variation and programming parameters modulate the resulting distribution. Treating each programming event as a sampling operation improves distribution expressiveness compared with read-based schemes, but at the cost of higher write energy and reduced endurance under repeated sampling, as storage and entropy generation rely on the same physical processes.


Together, these examples highlight why coupled pCIM architectures achieve high intrinsic efficiency and parallelism yet face inherent challenges in distribution programmability and long-term robustness. Because mean and variance are governed by shared device-level mechanisms, fine-grained and independent control remains limited, and frequent sampling can accelerate device wear\cite{Nature-communication}. These limitations motivate architectural approaches that decouple deterministic parameter storage from entropy generation, which we discuss next.

\begin{figurehere}
   \centering
    \includegraphics[width=1\linewidth]{bib/arch-comparison.png}
    \captionsetup{parbox=none} % for caption to be split
    \caption{xxxx}
    \label{fig:overview}
\end{figurehere}

\noindent\textbf{Decoupled Parameter Storage and Sampling}

\noindent  Decoupled probabilistic compute-in-memory architectures separate deterministic parameter storage from entropy generation, enabling probabilistic representations in which distribution parameters can be programmed independently. A common example is Gaussian sampling, where a probabilistic variable is expressed as the sum of a deterministic mean and a stochastic component scaled by an independently stored variance. By disentangling storage from sampling, decoupled pCIM avoids binding probabilistic behavior to a single device-level mechanism and instead exposes probability distributions as configurable, model-aligned primitives.


Existing decoupled pCIM designs can be broadly divided into near-memory and in-memory approaches. Near-memory implementations\cite{fpga_bnn,STT-MRAM_cim} place entropy generation close to, but outside, the memory array, reducing some data-movement overhead compared with conventional von Neumann pipelines while preserving modularity and distribution programmability. Although sampled values still traverse an explicit interface, this organization offers a pragmatic balance between flexibility and efficiency, particularly for early-stage or heterogeneous systems.


In-memory decoupled architectures integrate entropy generation within the memory array or its immediate periphery, allowing memory accesses to directly yield sampled values without explicitly materializing random numbers\cite{isscc_shot_noise,peiUncertaintyawareRoboticPerception2025a}. This approach aligns sampling with memory-level parallelism and offers a promising path toward scalable probabilistic execution. At the same time, realizing high-quality sampling at scale introduces important engineering considerations. In particular, probabilistic correctness often assumes sufficiently independent entropy sources, which can be challenged by systematic mismatch, spatial correlation, and process variation across large arrays. Addressing these effects may require calibration, testing, or architectural mitigation. In addition, embedding entropy sources and the supporting circuitry needed to combine stochastic terms with stored variance can impact memory density, motivating careful co-design to balance sampling capability and storage efficiency.


Overall, decoupled pCIM architectures substantially expand distribution programmability and compatibility with probabilistic learning models, addressing key limitations of coupled designs. The distinctions between near-memory and in-memory realizations highlight complementary trade-offs among entropy bandwidth, locality, density, and system complexity. Rather than fundamental obstacles, these factors define a rich design space in which architectural choices can be tailored to application requirements, underscoring the long-term potential of decoupled pCIM for scalable probabilistic workloads.

\noindent\textbf{pCIM as General-Purpose Memory}

\noindent  Across the five memory-level dimensions, both coupled and decoupled probabilistic compute-in-memory architectures elevate probabilistic data to first-class memory objects by integrating sampling with storage and access. Compared with von Neumann systems, both reduce data movement, expose memory-level parallelism, and allow probabilistic workloads to scale with memory bandwidth rather than serialized random number generation. Their differences lie in how these benefits are balanced. Coupled pCIM maximizes efficiency and parallelism by unifying parameter storage and sampling within the same device, but constrains distribution programmability and ties robustness to device-level variability. Decoupled pCIM separates storage from entropy generation, improving programmability and robustness while introducing additional circuitry, entropy management, and potential density overhead. Together, these trade-offs frame a clear design space between compact, efficiency-driven coupling and flexible, scalable decoupling within probabilistic memory systems.
\end{comment}

\noindent Artificial intelligence systems are increasingly deployed in high-stakes settings, including medical decision-making~\cite{metwallyPredictionMetabolicSubphenotypes2025}, autonomous platforms~\cite{automated_driving_nn,autonomous_driving_dl} and robotic agents~\cite{science_robotics_uhang,robot_embodied_ai_2021}. In these applications, reliable operation requires more than accurate prediction. Systems must also quantify uncertainty~\cite{isscc_shot_noise}, explain their decisions~\cite{nutiExplainableBayesianDecision2021} and protect sensitive information~\cite{davisInSituPrivacyMixedSignal2024}. Uncertainty is therefore not a peripheral disturbance, but a structural part of the problem. Inputs are noisy, environments evolve, and models remain imperfect or adversarially exposed. As a result, modern AI systems increasingly rely on probability and randomness to support trustworthy operation.

Stochastic sampling has long been a fundamental tool for working with probability and has co-evolved with computing platforms for more than eight decades. From classical Monte Carlo methods for estimating intractable quantities~\cite{Monte-Carlo}, early systems such as the MANIAC computer demonstrated Monte Carlo sampling for physical simulation~\cite{xxxx}. As computing platforms evolved from discrete vacuum tubes to modern integrated circuits and transistors, sampling-based methods expanded to more complex and dynamic settings, including particle filtering~\cite{xxxx} for time-varying inference and Monte Carlo Tree Search (MCTS)~\cite{xxxx} for large-scale decision making, enabled by increasing computational capability on CPUs. In parallel, techniques for random number generation evolved from software pseudo-random methods to high-throughput hardware entropy sources.

In modern AI workloads, sampling has become pervasive across a broad range of tasks. Bayesian and uncertainty-aware models rely on repeated sampling to characterize predictive uncertainty~\cite{peiUncertaintyawareRoboticPerception2025a}, generative models such as diffusion models produce outputs through iterative stochastic processes~\cite{cao_survey_2023}, interpretability methods leverage randomized perturbations to explain model behavior~\cite{ribeiro_lime_2016}, and privacy-preserving or secure systems introduce controlled randomness via noise injection and related mechanisms~\cite{davisInSituPrivacyMixedSignal2024}. Despite their diverse objectives, these approaches share a common computational pattern: the repeated generation and processing of random samples.

In the modern AI era, probabilistic computation increasingly interacts with large-scale neural networks executed on GPUs and specialized accelerators~\cite{google_tpu}. Although computing throughput has increased dramatically, improvements in memory density and bandwidth have been significantly slower~\cite{memory_wall_wulf}. This imbalance has exposed the well-known ``memory wall'' in modern AI systems, where data movement increasingly dominates the total energy and latency cost. To address this challenge, compute-in-memory (CIM) architectures have been explored to shift computation closer to the data source~\cite{cim_nature_sun_2023}. More recently, probabilistic compute-in-memory (p-CIM) approaches integrate stochastic functionality directly within memory structures by leveraging intrinsic device randomness~\cite{xxx}, enabling in-situ random number generation and probabilistic operations. Such architectures aim to reduce both sampling overhead and data movement for workloads such as Bayesian neural networks and uncertainty-aware models. Figure~\ref{fig:overview} summarizes this co-evolution across probabilistic algorithms, computing platforms, random number generation, and memory systems.


Prior reviews have examined probabilistic computation from several perspectives, including probabilistic algorithms~\cite{ghahramani_probabilistic_2015}, device-level randomness generation~\cite{xxxx}, and security mechanisms in compute-in-memory systems~\cite{wang_safe_2024}. In this Perspective, we focus instead on how probabilistic computation interacts with memory access and data movement. From this viewpoint, stochastic sampling can be interpreted as a form of generalized data access. Generating a random sample corresponds to reading data with a controlled probability distribution, while conventional deterministic memory access can be viewed as a special case with zero variance. This interpretation places random number generation and deterministic memory operations within a unified framework of data access primitives. It also suggests new directions for future memory architectures that can efficiently support entropy-intensive workloads in trustworthy AI systems.
